Combining Rules and Embeddings via Neuro-Symbolic AI for Knowledge Base Completion

Recent interest in Knowledge Base Completion (KBC) has led to a plethora of approaches based on reinforcement learning, inductive logic programming and graph embeddings. In particular, rule-based KBC has led to interpretable rules while being comparable in performance with graph embeddings. Even within rule-based KBC, there exist different approaches that lead to rules of varying quality and previous work has not always been precise in highlighting these differences. Another issue that plagues most rule-based KBC is the non-uniformity of relation paths: some relation sequences occur in very few paths while others appear very frequently. In this paper, we show that not all rule-based KBC models are the same and propose two distinct approaches that learn in one case: 1) a mixture of relations and the other 2) a mixture of paths. When implemented on top of neuro-symbolic AI, which learns rules by extending Boolean logic to real-valued logic, the latter model leads to superior KBC accuracy outperforming state-of-the-art rule-based KBC by 2-10% in terms of mean reciprocal rank. Furthermore, to address the non-uniformity of relation paths, we combine rule-based KBC with graph embeddings thus improving our results even further and achieving the best of both worlds.

==> sections/introduction.tex <==
\section{Introduction}

% Reasoning has been central to Artificial Intelligence research and knowledge is fundamental to most reasoning methods~\cite{}. One of the prominent ways to express knowledge is in the form of Knowledge Graphs, where nodes are entities and edge-labels are relationships that connect the entities. 
% %For example: Figure~\ref{fig:fact_example} shows the representation of the statement ``Joe Biden is the president of the United States of America" from DBpedia~\cite{}, an open knowledge graph comprising of millions of structured encyclopedic facts from Wikipedia. 
% Open knowledge graphs such as Wikidata~\cite{}, Yago~\cite{}, Nell~\cite{}, and subsets of Freebase~\cite{} have abundant information and are leveraged for various reasoning tasks~\cite{}. However, these knowledge graphs are inherently incomplete and there is recent surge in research methodologies to complete these knowledge graphs.        

%  In this work, we present a simple but effective, neuro-symbolic framework to combine rule-based learning with embeddings based approach to reap the best of both worlds.

\eat{Open knowledge graphs such as Wikidata~\cite{vrandevcic2014wikidata}, Yago~\cite{rebele2016yago}, NELL~\cite{carlson2010toward}, and subsets of Freebase~\cite{bollacker2008freebase} have abundant information and are leveraged for various reasoning tasks~\cite{}. 
However, these knowledge graphs are inherently incomplete. 
% and there is recent surge in research methodologies to complete these knowledge graphs. 
Rule learning techniques for knowledge base completion has gained significant attention in the recent past~\cite{sadeghian2019drum,minervini2020learning,yang2017differentiable}. These techniques learn multi-hop, first order logic rules that are interpretable and enables complex reasoning over knowledge graphs. For example, the rule $\forall X, Y nationality(X, Y) \rightarrow bornIn(X, Z) 	\land partOf(Z, Y)$, can be leveraged to infer the nationality of a person based on his place of birth and the country this place belongs to. }
% For example: -- Provide an example here --.
%Such first order logic rules are also easily transferable and does not require retraining given that the knowledge graphs are constantly updating.  

Open knowledge graphs (KG) such as Wikidata~\citep{vrandevcic2014wikidata}, Yago~\citep{rebele2016yago}, and Freebase~\citep{bollacker2008freebase} contain abundant information that is being leveraged for various reasoning tasks~\citep{kapanipathi:aclfindings2021}. However, such KGs are inherently incomplete. 
Consequently, a number of approaches have been proposed for knowledge base completion (KBC). Compared to knowledge graph embeddings, rule learning techniques for KBC harbor certain advantages such as 1) being able to handle newly added KG vertices whose embeddings may not be available, also referred to as the inductive setting \citep{yang:nips17,sadeghian:neurips19}, and 2) learning human-interpretable rules. These techniques learn multi-hop, first order logic rules that are interpretable which also enable complex reasoning over knowledge graphs. For example, the following rule (from Freebase) infers a person's nationality given her/his place of birth and the country of the birth place:
\begin{equation*}
\forall P,N ~ \exists L\!\!: \text{nationality}(P, N) \!\leftarrow \text{bornIn}(P,L) \land~ \text{partOf}(L,N)
\end{equation*}

\eat{Existing approaches for learning multi-hop/chains of predicates have primarily focused on: (a) mixture of predicates: for instance ~\cite{yang2017differentiable} uses gradient-based optimization for inductive logic programming task focusing on individual predicates; (b) mixture of paths: techniques based on reinforcement learning~\cite{das2017go, lin2018multi} and page rank~\cite{mazumder2017context} score relation sequences from the knowledge graph in order to learn first order logic rules for inferring new facts. In comparison to mixture of predicates, paths have shown to have worked better by restricting the search space to the meaningful combinations of relations existing in the knowledge graph. These approaches, however, are typically complex with many modules \cite{qu2020rnnlogic} and parameters to optimize \cite{}. Therefore, in this work, we use a conceptually simple but sophisticated  neuro-symbolic AI machinery called Logical Neural Networks (LNN) which allows expressing rules in real-valued logic.}

\begin{figure}
\begin{minipage}{0.55\linewidth}
{\scriptsize
\begin{tikzpicture}[>=latex]
 \node[rectangle,fill=blue!20] (rmix) at (0,0) {$R(U,V)$};
 \node (impl) at (0.8,0) {$\leftarrow$};
 \node[rectangle,fill=red!20] (fill1) at (1.6,0) {$\underline{?}(U,W)$};
 \node (conj) at (2.3,0) {$\wedge$};
 \node[rectangle,fill=red!20] (fill2) at (3,0) {$\underline{?}(W,V)$};
 
 \node (r1) at (0.8,-1) {$R_1$};
 \draw[->] (r1) -- (fill1);
 \node (r2) at (1.2,-1) {$R_2$};
 \draw[->] (r2) -- (fill1);
 \node (r3) at (1.6,-1) {$\ldots$};
 \draw[->] (r3) -- (fill1);
 \node (r4) at (2,-1) {$R_n$};
 \draw[->] (r4) -- (fill1);
 
 \node (r5) at (2.6,-1) {$R_1$};
 \draw[->] (r5) -- (fill2);
 \node (r6) at (3.0,-1) {$R_2$};
 \draw[->] (r6) -- (fill2);
 \node (r7) at (3.4,-1) {$\ldots$};
 \draw[->] (r7) -- (fill2);
 \node (r8) at (3.8,-1) {$R_n$};
 \draw[->] (r8) -- (fill2);
\end{tikzpicture}
}
\centerline{(a)}
\end{minipage}
\begin{minipage}{0.35\linewidth}
{\scriptsize
\begin{tikzpicture}[>=latex]
 \node[rectangle,fill=blue!20] (rmix) at (0,0) {$R(U,V)$};
 \node (impl) at (0.8,0) {$\leftarrow$};
 \node[rectangle,fill=red!20] (fill1) at (1.6,0) {$\underline{??}(U,V)$};
 
 \node (r2) at (-0.2,-0.4) {$\ldots$};
 \draw[->] (r2) -- (1.2,-0.4) -- (1.2,-0.2);
 \node (r3) at (-0.2,-0.7) {$R_i(U,W) \wedge R_j(W,V)$};
 \draw[->] (r3) -- (1.3,-0.7) -- (1.3,-0.2);
 \node (r4) at (-0.2,-1) {$\ldots$};
 \draw[->] (r4) -- (1.4,-1) -- (1.4,-0.2);
\end{tikzpicture}
}
\centerline{(b)}
\end{minipage}
\caption{Rule-based KBC approaches: (a) CPM, (b) MRP.}
\label{fig:ruletemplates}
\end{figure}

NeuralLP \citep{yang:nips17} was amongst the first to learn rules for KBC by using a mixture of all relations present in the KG to represent each relation appearing in the \emph{body} of the rule, i.e. appearing towards the right of the implication ($\leftarrow$ symbol in the previous example). DRUM \citep{sadeghian:neurips19} improves upon NeuralLP by proposing to learn multiple such rules each comprising mixtures of relations and also adds a low-rank tensor factorization scheme to keep the number of parameters in check. MINERVA \citep{das:iclr18} steps away from representing each body relation as a mixture, proposing instead to learn the relation sequences appearing in paths connecting source to destination vertices using neural reinforcement learning. RNNLogic \citep{qu:iclr21} is the latest to adopt such a path-based rule learning approach for KBC. It consists of two modules, a rule-generator for suggesting a \emph{set} of high quality paths and a reasoning predictor that uses said paths to predict missing information. To jointly train the two, RNNLogic employs expectation-maximization (EM) where the E-step identifies useful paths per data instance (edge in the KG) by sampling from an intractable posterior while the M-step uses the per instance useful paths to update the overall set of paths. Both DRUM and RNNLogic represent a significant increase in complexity of the approach compared to NeuralLP and MINERVA, respectively, so it is not surprising that they claim improvements in KBC quality but even this is not a given due to the choice of KBC evaluation metrics used by the aforementioned approaches.

\begin{table}
\caption{Fraction of reachable test set triples.}
\centering
{\scriptsize
\begin{tabular}{ccc}
\toprule
Path Length & WN18RR & FB15K-237\\
\midrule
1 & $0.35$ & $0.00$\\
2 & $0.44$ & $0.74$\\
3 & $0.66$ & $0.99$\\
4 & $0.73$ & $1.00$\\
5 & $0.82$ & $1.00$\\
\bottomrule
\end{tabular}
}
\label{tab:reachabledestinations}
\end{table}

Recently, \citet{sun:acl20} showed that certain gains reported on KBC benchmarks were caused not due to the improvements in neural network architecture employed, but due to these networks being prone to generating $0$ activations. A similar phenomenon can take place in rule-based KBC when learning rules of insufficient length (defined as the number of predicates in the body of the rule). Following previous works, we formalize the KBC task as that of predicting destinations: Given a query $\langle h, r, ? \rangle$ where $h$ and $r$ denote a source vertex and relation from the KG, the goal is to predict the destination vertex. \mytabref{tab:reachabledestinations} reports the fraction of test set triples of the form $\langle h, r, t \rangle$ in popular KBC benchmarks whose destination can be reached from the source via paths of varying length (defined as the number of edges in the path). In particular, in WN18RR only $44\%$ of test set's destinations can be reached from its corresponding sources using paths of up to length $2$. This implies that with rules of length up to $2$, one can only hope to attain a maximum Hits@10 of $0.44$ (attained when all reachable destinations are ranked within the top-$10$). However, Table 4 in DRUM \citep{sadeghian:neurips19} reports Hits@10 $=0.568 > 0.44$ with rules of length up to $2$. We conjecture that this happens when an unreachable destination is assigned a default score by the KBC approach, usually $0$, and by adopting the evaluation metrics proposed by \citeauthor{sun:acl20} one can detect such shortcomings in the KBC approach.
  
\par

Instead of following the current trend of devising increasingly complex rule-based KBC approaches, and given that previously published results may not be trustworthy, in this paper, our goal is to distill the prevalent rule-learning approaches down to their core ideas and compare them using coherent metrics. More precisely, we devise two approaches. The first approach, denoted \emph{Chain of Predicate Mixtures} (CPM), represents each relation in the body of the rule as a mixture and has close ties to NeuralLP, DRUM. The second approach, denoted \emph{Mixture of Relation Paths} (MRP), learns relation paths and has close ties to MINERVA, RNNLogic. \myfigref{fig:ruletemplates} depicts both CPM, MRP for learning a rule with two relations in the body. CPM forms two mixtures whereas MRP forms a mixture of all possible two relation paths. While the approaches are conceptually simple, we do however utilize powerful machinery. For both CPM and MRP, we propose to utilize \emph{Logical Neural Networks} (LNN) \citep{riegel:arxiv20} which is a powerful member of the neuro-symbolic AI (NeSy) family of approaches. LNN is an extension of Boolean logic to the real-valued domain and are differentiable thus enabling us to learn rules end-to-end via gradient-based optimization. While other members of NeSy harbor tenuous connections to Boolean logic's semantics, e.g., \citep{dong:iclr19}, LNN shares strong ties thus making the learned rules fully interpretable to humans. 
  
\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{kinship_rnnlogic.png}
    \caption{Path counts within cells are in thousands ($\times 1000$)}
    \label{fig:kinshipcounts}
\end{figure}  
  
One shortcoming of path-based rule learning, such as MRP, is that it suffers from the issue of sparsity. Since not all relation paths are equally prevalent in the KG, our goal is to guide the learning process towards more prevalent, effective relation paths as opposed to paths that appear less frequently. For instance, \myfigref{fig:kinshipcounts} depicts the distribution of all possible length $2$ paths with the first relation depicted along rows and the second relation depicted along columns in the Kinship \cite{kok2007statistical} benchmark. Barring four cells, all the other path counts are below $1000$ and vast majority are in single digits. Going beyond length $2$, the distribution becomes even more skewed. We show how to use pre-trained knowledge graph embeddings (KGE) to guide CPM and MRP to learn more effective rules in such a setting. While RNNLogic \citep{qu:iclr21} scores paths using a specific kind of KGE (RotatE~\cite{sun2019rotate}), we show how to use any of the vast array of KGEs available in the literature.

\eat{a rule consisting of a rare predicate $R$ (corresponding to fewer positive triples in the KB) simply will not have sufficient paths to reliably estimate model parameters. On the other hand, knowledge graph embeddings learn \emph{projection} operators \citep{ren:iclr20,ren:neurips20} based on neighborhood information which is abundant in comparison to paths between entities. However, combining rule-learning based approaches with such embedding-based techniques are rarely  been explored except~\citet{qu2020rnnlogic}. Therefore, inspired by~\citet{qu2020rnnlogic}{\color{red}Change this if necessary.}, we present a novel framework that can exploit the best of both rule-learning (LNN~\cite{riegel:arxiv20}) and embedding based approach (RotatE~\cite{sun2019rotate}). }
% Our experimental evaluation shows that our LNN-based approach achieves state-of-the-art performance on four standard benchmarks, and when combined with embedding techniques, the performance improves even further. 


\noindent Our contributions are: 
\squishlist
\item We propose to implement with logical neural networks (LNN) two simple approaches for rule-based KBC. LNN is a differentiable framework for real-valued logic that has strong connections to Boolean logic semantics.
\item To address the non-uniform distribution of relation paths that is likely to exist in any KG, we propose a simple approach that combines rule-based KBC with any KGE in order to reap the complementary benefits of both worlds.
\item Our experiments compare the proposed approaches with $6$ rule-based KBC baselines on $4$ different KBC benchmarks ($2$ of which have multiple splits). $3$ of the baseline implementations include unreliable metrics which we update with metrics based on \citet{sun:acl20}'s.
\item Our experimental results include:
\squishlisttwo
    \item MRP outperforms CPM in terms of KBC quality. However, the margin separating the two depends on the dataset.
    \item Simple MRP is comparable to SotA in rule-based KBC.
    \item We improve upon FB15k-237's rule-based KBC SotA leading to $2\%$ ($6.6\%$) improvement in mean reciprocal rank when used with (without) KGE.
\squishend
\squishend


%However, these techniques are complex ~\cite{}

%RNNLogic: so many modules? many parameters to optimize 
%Minerva: 

% Use of LNN is new
% A framework to incorporate any embeddings to a rule learning technique is new -- LNN
% 

%%% Learning chain FOL rules -- NeuralLP learning chain rules using one hop rules.
%%% Path-based 
%%% Path-based approaches work better but are complex. 
%% Comparison between these two approaches using LNN and found that latter works better. 

%% Sparsity issue 


%are They are inherently incomplete
%% There are primarily two class of techniques to complete knowledge bases via induction. (a) embedding based techniques, that learn translational embeddings or projections for different relations in the knowledge base~\cite{}; and (b) Rule-learning based techniques, that learn symbolic rules from the knowledge graph that can be used to infer other relations~\cite{}. 

% Both techniques can be complementary have their advantages (Be more specific here). However, leveraging the best of both worlds is yet to be well explored~\cite{RNNLogic}.  

%Embedding based techniques focuses on  While the performance of embeddings based techniques has shown to have improved significantly over time, tranditional rule-learning techniques have gained attention due to its inherent ability to be interpretable. 





%Prithvi comment: These are not really contributions. They are more of a summary/story. Felt like I needed to summarize the story so that we can follow and expand/add to it.
% Our contributions:
% \begin{itemize}
% \item Conceptual simplicity of the approach -- Sophisticated machinery using neuro-symbolic AI (LNNs). On top of this we learn rules that outperforms RL based approaches that are complex architecture. 

%     \item We devise two simple approaches for learning rules for KBC. Albeit simple, both approaches rely on sophisticated machinery, viz. logical neural networks \citep{riegel:arxiv20} which is a particularly powerful member of the neuro-symbolic AI family capable of expressing rules in real-valued logic. While the former approach expresses each predicate in the body of the rule as a mixture over all base \emph{predicates} available in the KB, the latter expresses the learned rule as a mixture over all possible \emph{paths} (restricted to a user-defined length).
%     \item We show empirically that while the second approach is more computationally expensive, it does lead to significantly better KBC performance as measured over standard benchmarks.
    % \item One shortcoming of the second approach is that it suffers from the issue of sparsity. Since not all predicates are equally prevalent in the base KB, a rule consisting of a rare predicate $R$ (corresponding to fewer positive triples in the KB) simply will not have sufficient paths for us to reliably estimate model parameters.
    % \item We introduce multiple approaches to overcome the sparsity issue. One of our more interesting proposals relies on a subclass of knowledge graph embeddings offering \emph{projection} operators \citep{ren:iclr20,ren:neurips20} which can help guide the rule-learning process towards a model that includes paths present in sufficient numbers in the training graph so as to allow us to reliably estimate model parameters.
    % \item Our experiments on standard benchmarks show that by combining rules and embeddings we can improve KBC performance over just rules or just embeddings leading to state-of-the-art results over commonly used benchmarks.
% \end{itemize}Conceptual simplicity of the approach -- Sophisticated machinery using neuro-symbolic AI (LNNs). On top of this we learn rules that outperforms RL based approaches that are complex architecture. 





==> sections/related_work.tex <==

\section{Related Work}
Knowledge Base Completion (KBC) approaches can primarily categorized into the three  classes: (a) embeddings-based techniques, (b) symbolic/logical rule learning techniques, (c) combination of rule-learning and embeddings. 

%% Embedding based approaches
Embeddings based techniques maps entities and relations to low-dimensional vector space to infer new facts. These techniques uses neighborhood structure of an entity or relation for learning embeddings. Starting off with translational embeddings~\cite{bordes2013translating}, embedding-based techniques have evolved to use complex vector spaces~\cite{survey} such as ComplEx~\cite{trouillon2016complex}, RotatE~\cite{sun2019rotate}, and QuatE~\cite{zhang2019quaternion}. 
% These techniques while showing very promising performance in predicting missing links in knolwedge bases, they are uninterpretable and incapable of generating rules that be used further used for other reasoning tasks {\color{red}add example}.

%% Rule learning
While the performance of embeddings based techniques has shown to have improved significantly over time, tranditional rule-learning techniques have gained attention due to its inherent ability to be generate interpretable rules ~\cite{yang2017differentiable,sadeghian2019drum,rocktaschel2017end, qu2020rnnlogic}. 
% The second category includes techniques which aim at learning interpretable rules over from a knowledge base. 
% Various existing methodologies such as path ranking algorithms~\cite{mazumder2017context}, reinforcement learning~\cite{das2017go, lin2018multi}, and inductive logic programming~\cite{} are used to learn rules to infer relations between entities in knowledge graphs. Techniques that rely on Path Ranking and Reinforcement Learning are path-based where paths existing in the knowledge graphs are scored for inference. 
These approaches try to learn symbolic rules which can be used infer other relations between entities the in knowledge graph. 
NeuralLP \cite{yang2017differentiable} is a fully differentiable rule learning approach based on TensorLog \cite{cohen2016tensorlog}, where the parameters and the structure of logic rules can be trained end-to-end with gradient based learning. Unlike NeuralLP and similar approaches\cite{sadeghian2019drum,rocktaschel2017end}, RNNLogic \cite{qu2020rnnlogic} separates rule generation from rule weight learning by introducing two separate modules, a rule generator to produce high-quality rules and a reasoning predictor that learns the weights of these rules.  These approaches, however, are fairly complex with many components and parameters to optimize. On the other hand, \sysname\ leverage a powerful neuro-symbolic approach (LNN), a simple yet poweful AI machinary, that learns logic rules in knowledge bases.  {\color{red}quantify simplicity} 


% %%%%% Reinforcement Learning based
% ~\citet{deepwalk} 
% ~\citet{das:iclr18} 
% ~\citet{lin2018multi}

%%%% NeuraLP and RNNLogic

%%% Why our approach is different to these

Complementary to embedding-based approaches that are optimized to leverage entity neighborhood information, rule-learning based approaches focus on multi-hop, compositions of relations in the knowledge-base and hence enabling complex, interpretable reasoning to derive new facts~\cite{multihoplin2019}. In this category, RNNLogic is the only system that investigated this powerful combination. Similar to RNNLogic, \sysname\ is also capable of utilizing knowledge graph embeddings for rule learning. We also showed emperically that this combination has led to performance gains over multiple KBC datasets. {\color{red} mention how we are different from RNNLogic, perhaps our flexibility to integrate multiple embedding methpds?}

% Our LNN-based approach falls in this category of approaches. 


% Both classes of approaches use complementary information from the knowledge graph but have been mostly explored independently of each other.


% \noindent \textbf{Knowledge Graph Embedding} 
% %KGE techniques -- learning simple implicit rules  
% %TransE bordes2013translating 
% %RotatE sun2019rotate
% %trouillon2016complex
% % ComplEx-N lacroix2018canonical

% \noindent \textbf{Rule Learning} 
% %Neural methods for rule learning that do not use embedding: DRUM, NeuralLP
% %NeuralLP yang2017differentiable
% %DRUM sadeghian2019drum 
% %CTP minervini2020learning

% \noindent \textbf{Rule Learning with embedding} 
% %Neural methods that use embedding: RNNLogic and us
% %rnnlogic qu2020rnnlogic

